Towards Rich, Portable, and Large-Scale Pedestrian Data Collection

Recently, pedestrian behavior research has shifted towards machine learning based methods and converged on the topic of modeling pedestrian interactions. For this, a large-scale dataset that contains rich information is needed. We propose a data collection system that is portable, which facilitates accessible large-scale data collection in diverse environments. We also couple the system with a semi-autonomous labeling pipeline for fast trajectory label production. We further introduce the first batch of dataset from the ongoing data collection effort -- the TBD pedestrian dataset. Compared with existing pedestrian datasets, our dataset contains three components: human verified labels grounded in the metric space, a combination of top-down and perspective views, and naturalistic human behavior in the presence of a socially appropriate "robot".

==> Related_Works.tex <==
\section{Related Work}

\label{sec:related-dsetuse}
As is expected from the explosion of data-hungry machine learning methods in robotics, demand for pedestrian datasets has been on the rise in recent years. One popular category of research in this domain is human trajectory prediction (e.g., \cite{Alahi1, Gupta1, Sophie, Social-STGCNN, ivanovic-trajectron, kitani-2012, liang2020garden, wang-split-merge}). Much of this research utilizes selected mechanisms to model pedestrian interactions in hopes for better prediction performance (e.g., pooling layers in the deep learning frameworks \cite{Alahi1, Gupta1} or graph-based representations \cite{Social-STGCNN}). Rudenko et al. \cite{rudenko2019-predSurvey} provides a good summary into this topic. While the state-of-the art performance keeps improving with the constant appearance of newer models, it is often unclear how well these models can generalize in diverse environments. As shown in \cite{rudenko2019-predSurvey}, many of these models only conduct their evaluation on the relatively small-scale ETH \cite{ETH} and UCY \cite{UCY} datasets.

Another popular demand for pedestrian datasets comes from social navigation research. Compared to human motion prediction research, social navigation research focuses more on planning. For example, social navigation research uses learning-based methods to identify socially appropriate motion for better robot behavior, such as deep reinforcement learning \cite{Everett18_IROS, chen2019crowd, Chen-gaze-learn} or inverse reinforcement learning \cite{okal-IRL, Tai-IRL}. Due to the lack of sufficiently large datasets, these models often train in simulators that lack realistic pedestrian behavior. Apart from training, datasets are also increasing in popularity in social navigation evaluation due to their realistic pedestrian behavior \cite{gao2021evaluation}. Social navigation methods are often evaluated in environments using pedestrian data trajectory playback (e.g., \cite{trautmanijrr, cao2019dynamic, sun2021move, wang2022group}). However, similar to human motion prediction research, these evaluations are typically only conducted on the ETH \cite{ETH} and UCY \cite{UCY} datasets as shown by \cite{gao2021evaluation}. These two datasets only use overhead views, and therefore lack the perspective view used by most robots. Comparisons between an intial dataset from our data collection system and existing datasets can be found in section \ref{sec:eval-compare}.



% \subsection{Simulators and Pedestrian Datasets} \label{sec:related-sim-dset}

% Simulators can fill in the role of datasets for both training and evaluation. Simulators such as PedSIM \cite{gloor2016pedsim}, CrowdNav \cite{chen2019crowd}, SocNavBench \cite{biswas2021socnavbench} and SEAN \cite{tsoi2020sean} are in use by the research community. However, sim-to-real transfer is an unsolved problem in robotics. Apart from lack of fidelity in visuals and physics, pedestrian simulators in particular entail the additional paradox of pedestrian behavior realism \cite{mavrogiannis2021core}: If pedestrian models are realistic enough for use in simulators, why don't we apply the same model to social navigation?

% In contrast, naturalistic datasets provide realistic pedestrian behavior. Unfortunately, datasets are limited in quantity, unlike simulators that can generate infinite pedestrian scenes. As mentioned in section \ref{sec:related-dsetuse}, most research is still limited to only the ETH and UCY datasets, which are small in scale and lack perspective views. Therefore, such datasets have an additional downside in that pedestrians do not react to the robot. While perspective views can be simulated using inferred laser scans from point perspectives (e.g., \cite{wang-split-merge}), this does not fill the need for camera data from perspective views. Also note that tying the simulated laser scanner location to a moving pedestrian in the data set will likely have unwanted noise in the human tracking. 


